Elle: Inferring Isolation Anomalies from Experimental Observations

Users who care about their data store it in databases, which (at least in principle) guarantee some form of transactional isolation. However, experience shows [Kleppmann 2019, Kingsbury and Patella 2019a] that many databases do not provide the isolation guarantees they claim. With the recent proliferation of new distributed databases, demand has grown for checkers that can, by generating client workloads and injecting faults, produce anomalies that witness a violation of a stated guarantee. An ideal checker would be sound (no false positives), efficient (polynomial in history length and concurrency), effective (finding violations in real databases), general (analyzing many patterns of transactions), and informative (justifying the presence of an anomaly with understandable counterexamples). Sadly, we are aware of no checkers that satisfy these goals. We present Elle: a novel checker which infers an Adya-style dependency graph between client-observed transactions. It does so by carefully selecting database objects and operations when generating histories, so as to ensure that the results of database reads reveal information about their version history. Elle can detect every anomaly in Adya et al's formalism [Adya et al. 2000] (except for predicates), discriminate between them, and provide concise explanations of each. This paper makes the following contributions: we present Elle, demonstrate its soundness, measure its efficiency against the current state of the art, and give evidence of its effectiveness via a case study of four real databases.

==> acks.tex <==
We wish to thank Kit Patella for prototyping early versions of our cycle detection checker, and Zach Tellman for his non-stack-consuming implementation of Tarjan’s algorithm [16]. PingCAP, the makers of TiDB, provided funding for their Jepsen analysis; part of this research was conducted as a part of that contract.

\paa{I want to thank Asha too}

==> attic.tex <==
Now consider a traceable $x$, and the sequence of versions $S_x = [x_{init} \ldots x_{max}]$ given by the trace of $x_{max}$.

\begin{lemma}
\label{version-order-subsequence-of-max-trace}
If $x$ is a traceable object, the sequence of versions given by $\ll$ is a subsequence of $S_x$.
\end{lemma}



This allows us to infer the order of versions in $\ll$ from the installed versions in $S_x$, and vice versa.

Can we derive $\ll_x$ from any version of $x$? Unfortunately no, but given an installed version of $x$, we can derive a chain which is a \textit{prefix} of $\ll_x$. By "the prefix of $\ll$ up to and including $x_i$, we mean the chain (a set of elements, plus a total order over them), derived from $\ll$, but without those elements $x_j$ such that $x_i \ll x_j$.\footnotemark

\footnotetext{Representing the order of transactions as a chain, rather than simply an order, simplifies the proof for single-element prefixes.}

==> completeness.tex <==
For completeness, we would like to show that if interpretations of an observation exist, and every interpretation of an observation contains a dirty update, or an aborted read, that we can detect those conditions using the above lemmata. We prove the contrapositive by taking an observation $O$ in which we *cannot* detect a dirty update or aborted read, and showing either that no interpretations exist, or that there exists some interpretation $(H, R)$ with transactions $\hat{T}$, event order $\hat{E}$, and version order $\ll$.

To simplify our argument, we assume that our updates are *pre-version-return-invariant*, in the sense that given an update $w(x_i, a) \xrightarrow{} (x_j, r)$, the return value $r$ does not depend on the pre-version $x_i$. This allows us to apply updates in any order.

Since $O$ has no detectable aborted reads or dirty updates, we know that $O$ must be consistent, and that it contains no aborted writes which are present in the trace of a committed read.

To construct the set of transactions $T$, we take the observed transactions $\hat{T}$, where every indeterminate transaction whose write is visible to some committed read is considered committed. Other indeterminate transactions may be either committed or aborted in $T$. This ensures $T$ is complete. Since $O$ has no aborted writes in the trace of a committed read, and since all *indeterminate* (in $\hat{T}$) updates in the trace of a committed read are considered committed in $T$, $T$ has no aborted updates in the trace of a committed read. $H$ therefore contains no aborted reads.

Since our objects are traceable, we can reconstruct the total order of versions and update operations which led to any read version. Given an object $x$ with longest committed read $x_{longest}$, we define an *fixed* update as one which must fall in the trace of $x_{longest}$. Other updates of $x$ are *unfixed*. The trace of $x_{longest}$ provides us with a total order over fixed updates on $x$. If the trace of $x_{longest}$ contains updates not in $T$, then no interpretation can exist; perhaps the database returned garbage values. Otherwise, we continue.

Any unfixed updates on $x$ must not occur in $x_{longest}$ by definition, which also implies they are never observed by a committed read. Uncommitted unfixed updates may be applied freely anywhere in the version graph. Committed unfixed updates must fall in some trace from $x_{longest}$ to $x_{max}$, in order to ensure $\ll$ is total over committed versions. $\ll$ is simply the union of the orders of committed versions in the traces of $x_{max}$, $y_{max}$, etc.

Our choice of where to apply unfixed updates can determine whether $H$ exhibits dirty updates. For instance, if we apply an aborted update to $x_{longest}$, then a committed update to that resulting state, we will have constructed an aborted read. However, so long as our updates are pre-version-return-invariant, we are free *not* to do this. Instead, we can apply all committed updates to $x$ immediately following $x_{longest}$, and apply aborted updates anywhere else---e.g. to the initial state.

TODO: Every read state has to be reachable somehow, right? How do we make sure that happens? And what's reachable depends on what you consider committed vs uncommitted, and the choice of committed vs uncommitted impacts where you can place things... blegggh




??? a miracle occurs ???

\begin{lemma}
\label{consistent+no-aborted-write-before-read}
If $O$ is a consistent observation, and there exists no aborted write $w(x_i, a) \xrightarrow{} (x'_i)$ and a committed read $r(x_j)$ in $O$, such that the trace of $x_j$ implies $x'_i <= x_j$, the pessimistic interpretation of $O$ (should it exist) is free of dirty updates and aborted reads.
\end{lemma}

\begin{proof}
Since $O$ is consistent, every committed read of some object $x$ observes a version along the trace $S$ of $x_{longest}$. The pessimistic interpretation of $O$ follows $S$ with a sequence of all remaining known-committed (e.g. committed in $O$) writes. All other writes are attached to the initial state $x_{init}$.

Can a version $x'_i$ in $S$ be aborted? We consider three cases for the transaction $\hat{T}$ in $O$ whose corresponding transaction $T$ in $H$ wrote $x'_i$.

\begin{enumerate}
    \item $\hat{T}$ is committed. $x_i$ is not aborted, by definition.
    \item $\hat{T}$ is indeterminate. Since $x'_i$ is in $S$, the pessimistic interpretation considers $T$ committed, and $x_i$ is not aborted, by definition.
    \item $\hat{T}$ is aborted. Then we know there exists an aborted write $w(x_i, a) \xrightarrow{} (x'_i)$, observed by the committed read of $x_{longest}$; a contradiction.
\end{enumerate}

Since every version in $S$ is committed, and committed reads always observe a version in $S$, $H$ is free of aborted reads. The only other committed versions in $H$ are those we applied linearly after $S$, which implies every version in the trace of $x_{max}$ is committed; no aborted write appears in or after $S$. This implies $H$ exhibits no dirty updates.
\end{proof}

\begin{theorem}
Given any observation $O$, we can prove whether a.) no interpretation of $O$ exists, b.) every interpretation of $O$ exhibits aborted read, c.) every interpretation of $O$ exhibits dirty update, d.) either b or c, or e.) there are interpretations of $O$ which do not exhibit dirty updates or aborted reads.
\end{theorem}

\begin{proof}
If we are unable to construct an event order $E$ from $\hat{T}$ and $\hat{E}$, then no interpretations exist. If $O$ is inconsistent, lemma \ref{inconsistent->aborted-read} implies every interpretation of $O$ exhibits aborted read. If $O$ contains a known-aborted write whose effects are reflected in a committed read, lemma \ref{consistent+aborted-write-before-read->dirty-update-or-aborted-read} implies every interpretation of $O$ exhibits dirty updates or aborted reads, and we can show, in some cases, exactly which. Otherwise, lemma \ref{consistent+no-aborted-write-before-read} implies at least one interpretation has neither dirty updates nor aborted reads.
\end{proof}


==> proof.tex <==
\subsection{Objects, Operations, Databases}

An \textit{object} $x$ is a mutable datatype: a set of \textit{versions}, written $x_i$, $x_j$, etc., an \textit{initial version}, labeled $x_{init}$, and a set of \textit{object operations}.

An object operation represents a state transition between two versions $x_i$ and $x_j$ of some object $x$. Object operations take an argument $a$ and produces a return value $r$. Formally, an operation like $w$ is a 5-tuple of objects, pre-versions, arguments, post-versions, and return values, but for clarity, we write $w(x, x_i, a) \xrightarrow{} (x_j, r)$. Where the object, argument, return value, or return tuple can be inferred from context or are unimportant, we may omit them, e.g. $w(x_i, a) -> (x_j)$, $w(x_i)$, $w(x_i) \xrightarrow{} (x_j)$, etc.

Like Adya, we consider two types of operations: reads and writes. A \textit{read} $r$ takes no argument, leaves the version of the object unchanged, and returns that version: $r(x_i, nil) \xrightarrow{} (x_i, x_i)$.

A write operation $w$ changes a version somehow.\footnotemark Write semantics are object-dependent. Adya's model (like many papers on transactional databases) assumes objects are registers, and that writes blindly replace the current value. Our other three objects incorporate increasingly specific dependencies on previous versions. Our proof is primarily concerned with objects like list append, but we provide definitions for the first three objects as illustrative examples.

\footnotetext{One could, of course, perform a write which leaves the version unchanged.}

\begin{figure*}[ht]
\label{fig:example-objects}
\begin{tabular}{l l l l}
 Object & Versions & $x_{init}$ & Writes \\
\hline
 Register   & Any       & nil  & $w(x_i, a) \xrightarrow{} (a, nil)$ \\
 Counter    & Integers  & 0    & $w(x_i, a) \xrightarrow{} (x_i+a, nil)$ \\
 Set Add    & Sets      & \{\} & $w(x_i, a) \xrightarrow{} (x_i \cup \{a\}, nil)$ \\
 List Append & Lists    & []   & $w([e_1, \ldots, e_n], a) \xrightarrow{} ([e_1, \ldots, e_n, a], nil)$ \\
\end{tabular}
\caption{Example objects.}
\end{figure*}

The versions and write operations on an object $x$ together yield a \textit{version graph} $v_x$: a directed graph whose vertices are versions, and whose edges are write operations labeled by their respective arguments.

A \textit{database} is a set of named objects $x$, $y$, etc.


\subsection{Transactions}

A \textit{transaction} is a list (a totally ordered set) of object operations, followed by at most one \textit{commit} or \textit{abort} operation. We say a transaction is \textit{committed} if it ends in a commit, and \textit{aborted} if it ends in an abort. We call the version resulting from a transaction's last write to object $x$ its \textit{final version} of $x$; any other writes of $x$ result in \textit{intermediate versions}. If a transaction commits, we say it \textit{installs} all final versions; we call these \textit{installed versions}. Diverging from Adya, we use \textit{committed versions} to refer to versions written by committed transactions, including intermediate versions. Versions from transactions which did not commit are called \textit{uncommitted versions}.

The initial version of every object is considered committed.

\subsection{Histories}

Per Adya et al, a \textit{history} $H$ comprises a set of transactions $T$ on objects in a database $D$, a partial order $E$ over operations in $T$, and a version order $\ll$ over versions of the objects in $D$.

The event order $E$ has the following constraints:

\begin{itemize}
    \item It preserves the order of all operations within a transaction, including commit or abort events.
    \item One cannot read from the future: if a read $r(x_i)$ is in $E$, then there must exist a write $w \xrightarrow{} (x_i)$ which precedes it.
    \item Transactions observe their own writes: if a transaction $T$ contains $w(x_i)$ followed by $r(x_j)$, and there exists no $w(x_k)$ between the write and read of $x_i$ in $T$, $x_i = x_j$.
    \item The history must be complete: if $E$ contains a read or write operation for a transaction $T_i$, $E$ must contain a commit or abort event for $T_i$.
\end{itemize}

The version order $\ll$ has two constraints, per Adya et al:

\begin{itemize}
    \item It is a total order on committed versions of each individual object; there is no ordering of objects written by uncommitted or aborted transactions.
    \item The version order for each object $x$ (which we write $\ll_x$) begins with the initial version $x_{init}$.
\end{itemize}

Driven by the intuition that the version order should be consistent with the order of operations on an object, that $x_i \ll x_j$ means $x_j$ overwrote $x_i$, and that cycles in $\ll$ are meant to capture anomalies like \textit{circular information flow}, we introduce an additional constraint: the version order $\ll$ should be consistent with the version graphs $v_x$, $v_y$, \ldots.

\begin{axiom}
\label{version-order->version-graph}
If $x_i \ll x_j$, there exists a path from $x_i$ to $x_j$ in $v_x$.
\end{axiom}

Since Adya's formalism uses registers, their version graphs are \textit{totally connected}: any version can be replaced with any other version in a single write. Axiom \ref{version-order->version-graph} is therefore trivial for registers, and need not be stated. For more complex datatypes, we believe this constraint is warranted: it would be odd if one appended 3 to the list $[1, 2]$, obtaining $[1, 2, 3]$, and yet the database believed $[1, 2, 3] \ll [1, 2]$.

\subsection{Dependencies}

We define four classes of direct dependencies between transactions. Three are taken directly from Adya et al, and the fourth is useful when writes cannot be related to reads.

\begin{itemize}
    \item \textbf{Direct write-write dependency}. A transaction $T_j$ \textit{directly ww-depends} on $T_i$ if $T_i$ installs a version $x_i$ of $x$, and $T_j$ installs $x$'s next version $x_j$, by $\ll$.
    \item \textbf{Direct write-read dependency}. A transaction $T_j$ \textit{directly wr-depends} on $T_i$ if $T_i$ installs some version $x_i$ and $T_j$ reads $x_i$.\footnotemark{}
    \item \textbf{Direct read-write dependency}. A transaction $T_j$ \textit{directly rw-depends} on $T_i$ if $T_i$ reads version $x_i$ of $x$, and $T_j$ installs $x$'s next version in $\ll$.
    \item \textbf{Direct read-read dependency}. A transaction $T_j$ \textit{directly rr-depends} on $T_i$ if $T_i$ reads version $x_i$ of $x$, and $T_j$ reads $x$'s next version in $\ll$.
\end{itemize}

\footnotetext{It appears that Adya et al's read dependencies don't rule out a transaction depending on itself. We preserve their definitions here, but assume that in serialization graphs, $T_i \neq T_j$.}

In Adya et al's formalism, rr-depends is redundant: any rr-dependency implies an rw-dependency followed by a wr-dependency. We mention it here because for some objects, like counters, it may be the most useful dependency we can infer.

A \textit{Direct Serialization Graph}, or \textit{DSG}, is a graph of dependencies between transactions. The DSG for a history $H$ is denoted DSG($H$). If $T_j$ ww-depends on $T_i$, there exists an edge labeled \textit{ww} from $T_i$ to $T_j$ in DSG(H), and similarly for wr- and rw-dependencies. One could construct alterate serialization graphs involving other dependencies, such as read-read dependencies, process orders, or realtime orders, but we leave those as an exercise to the reader.

\subsection{Dirty Updates}

Consider what happens when a write $w$ takes one version $x_i$ to another $x_j$. In an ideal database, both versions are committed: $x$ reflects a totally ordered sequence of committed writes. Of course, $w$ might \textit{not} commit, in which case $x_j$ is not a committed version. This is fine; transactions abort all the time. What if, on the other hand, $x_i$ is uncommitted, and $w$ commits?

This is the write analogue to Adya et al's \textit{aborted read}, and both are possible under our definition of a history. $\ll$ orders pairs of committed versions, so $x_i$ is not comparable to $x_j$ in $\ll$, but $x_i$ \textit{can} precede $x_j$ in the version graph $v_x$. The effects of uncommitted transactions may "leak" into committed state, and be visible to later reads. This is (we believe) bad.

Adya defines \textit{G1a: Aborted Read} as a committed transaction $T_2$ containing a read of some value $x_i$ which was written by an aborted transaction $T_1$. However, this definition does not address our issue: in Adya's model, writes have no dependence on previous versions, so overwriting an uncommitted version is perfectly legal (so long as that uncommitted version was never read).

We therefore define a complementary phenomenon to G1a, intended to cover scenarios in which information leaks from uncommitted versions to committed ones. A history exhibits \textit{Dirty Update} if it contains an uncommitted transaction $T_1$ which writes $x_i$, and a committed transaction $T_2$, which contains a write acting on $x_i$.


\subsection{Traceable Objects}

Recall that for an object $x$, the version graph $v_x$ is comprised of versions connected by object operations. We call a path in $v_x$ from $x_{init}$ to some version $x_i$ a \textit{trace} of $x_i$.

We say $x$ is \textit{traceable} if every version $x_i$ has exactly one trace; i.e. $v_x$ is a tree. As a tree, $v_x$ is also acyclic.

\begin{lemma}
\label{traceable->x_max-trace-all-committed}
If $x$ is a traceable object in a history $H$, every committed version of $x$ is in the trace of $x_{max}$.
\end{lemma}

This follows from axiom \ref{version-order->version-graph}, and the fact that the version order $\ll$ is total over installed versions.

\begin{lemma}
\label{list-append-is-traceable}
List append objects are traceable.
\end{lemma}

Because list append appends the argument for each write to the end of the previous value, the sequence of write arguments up to some $x_i$ is exactly the sequence of elements in $x_i$.


\subsection{Version Orders and Version Graphs}

Let $x$ be an object in some version order $\ll$. We call the largest version of $x$, by $\ll$, $x_{max}$. Now consider a traceable $x$, and the sequence of versions $S_x = [x_{init} \ldots x_{max}]$ given by the trace of $x_{max}$.

\begin{lemma}
\label{version-order-subsequence-of-max-trace}
If $x$ is a traceable object, the sequence of versions given by $\ll$ is a subsequence of $S_x$.
\end{lemma}

\begin{proof}
Since $\ll$ starts with $x_{init}$ and ends with $x_{max}$, axiom \ref{version-order->version-graph} implies there exists a path $P_x$ from $x_{init}$ to $x_{max}$ whose versions are a supersequence of $\ll$. Since $x$ is traceable, there is exactly one such path: $S_x$. Therefore, $P_x = S_x$, which implies $\ll$ is a subsequence of $S_x$.
\end{proof}

This allows us to infer the order of versions in $\ll$ from the installed versions in $S_x$, and vice versa.

Can we derive $\ll_x$ from any version of $x$? Unfortunately no, but given an installed version of $x$, we can derive a chain which is a \textit{prefix} of $\ll_x$. By "the prefix of $\ll$ up to and including $x_i$, we mean the chain (a set of elements, plus a total order over them), derived from $\ll$, but without those elements $x_j$ such that $x_i \ll x_j$.\footnotemark

\footnotetext{Representing the order of transactions as a chain, rather than simply an order, simplifies the proof for single-element prefixes.}

\begin{lemma}
\label{x_i->ll_x-prefix}
If $x_i$ is an installed version of a traceable object $x$, removing intermediate and aborted versions from the versions in the trace of $x_i$ yields the prefix of $\ll_x$ up to and including $x_i$.
\end{lemma}

The version order for $x$, $\ll_x$, provides a total order of installed (e.g. non-intermediate and non-aborted) versions of $x$. Per axiom \ref{version-order->version-graph}, $v_x$ has a path which connects those versions, possibly via intermediate and/or aborted versions. Thanks to traceability, that path is unique, and must be $S_x$.


\subsection{Observations}

Imagine a set of singlethreaded logical processes which interact with a database system as clients. Each process submits transactions for execution and receives information about the return values of the operations in those transactions. What can we tell from the perspective of those client processes?

Recall that an object operation has five components: $w(x, x_i, a) \xrightarrow{} (x_j, r)$ denotes a write to object $x$ which takes version $x_i$ and combines it with argument $a$ to yield version $x_j$, returning $r$. When a client makes a write, it knows the object $x$ and argument $a$, but (likely) not the versions $x_i$ or $x_j$. If the transaction commits, the client may know the return value $r$, but might not if, for example, a response message is lost by the network.

We define an \textit{observed object operation} as an operation whose versions and return value may be unknown. We write observed operations with a hat: $\hat{w}(x, \_, 3) \xrightarrow{} (\_, nil)$ denotes an observed write of 3 to object $x$, returning $nil$; the versions involved are unknown.

An \textit{observed operation} is either an observed object operation, a commit, or an abort.

An \textit{observed transaction}, written $\hat{T_i}$, is a transaction composed of observed operations. If a client attempts to abort, or does not attempt to commit, a transaction, the observed transaction ends in an abort. If a transaction is known to have committed, it ends in a commit operation. However, when a client \textit{attempts} to commit a transaction, but the result is unknown, e.g. due to a timeout or database crash, we leave the transaction with neither a commit nor abort operation.

An \textit{Observation} $O$ represents the experimentally-accessible information about a database system's behavior. Observations have a set of observed transactions $\hat{T}$. We assume observations include every transaction executed by a database system.

We say that O is \textit{determinate} if every transaction in $\hat{T}$ is either committed or aborted; e.g. there are no indeterminate transactions. Otherwise, $O$ is \textit{indeterminate}.




\subsection{Interpretations}

Consider an operation $o = f(x_i, a) \xrightarrow{} (x_j, r)$ and an observed operation $\hat{o} = \hat{f}(\hat{x_i}, \hat{a}) \xrightarrow{} (\hat{x}_j, \hat{r})$. We say that $o$ is \textit{compatible with} $\hat{o}$ iff:

\begin{itemize}
    \item $f = \hat{f}$
    \item $a = \hat{a}$
    \item $\hat{r}$ is either \textit{unknown} or equal to $r$
    \item $\hat{x_i}$ is either \textit{unknown} or equal to $x_i$
    \item $\hat{x}_j$ is either \textit{unknown} or equal to $x_j$
\end{itemize}

Intuitively, an "abstract" operation $o$ is compatible with an observed operation $\hat{o}$ if the two execute the same type of operation (e.g. a read) on the same key with the same argument, and their return values and versions don't conflict---that is, $\hat{o}$ could have been an observation of $o$.

Now consider a transaction $T_i$ and an observed transaction $\hat{T_i}$. We say that $T_i$ is \textit{compatible with} $\hat{T_i}$ iff:

\begin{itemize}
    \item They have the same number of object operations.
    \item Every object operation in $T_i$ is compatible with its corresponding object operation in $\hat{T_i}$.
    \item If $T_i$ committed, $\hat{T_i}$ is not aborted, and if $\hat{T_i}$ committed, $T_i$ committed too.
    \item If $T_i$ aborted, $\hat{T_i}$ is not committed, and if $\hat{T_i}$ aborted, $T_i$ aborted too.
\end{itemize}

Finally, consider a history $H$ and an observation $O$, with transactions $T$ and $\hat{T}$ respectively. We say that $H$ is \textit{compatible with} $O$ iff $H$ is complete, and there exists a bijection $R$ from $\hat{T}$ to $T$ such that $\forall (\hat{T_i}, T_i) \in R, T_i \textrm{ is compatible with } \hat{T_i}$. We call a choice of $(H, R)$ which satisfies this constraint an \textit{interpretation} of $O$. Given an interpretation, we say that $T_i = R \hat{T}_i$ is the \textit{corresponding transaction} to $\hat{T_i}$, and vice versa.

Intuitively, given transactions observed by clients, we may interpret that behavior as the result of any number of histories. In such an interpretation, every observed transaction corresponds to a distinct abstract transaction in the history, taking into account that we may not know exactly what versions or return values were involved, or whether or not observed transactions actually committed. These definitions of \textit{compatible} formalize an intuitive "theory of mind" for a database: what we think could be going on behind the scenes.

There may be many histories compatible with a given observation. For instance, an indeterminate observed transaction may either commit or abort in a compatible history. Given two identical increment transactions, there are two choices of R for any history H, since the two are interchangeable. There may also be many observations compatible with a given history: for instance, we could observe a transaction's commit, or fail to observe it, and label it indeterminate.



\subsection{Recoverability}

Given an observation, we would like to infer relationships between observed transactions. Which transaction wrote $x_i$? Which transaction read $x_i$?

For reads, this is straightforward. The definition of a read (TODO: enforce completeness of return values in committed txns in observations) requires that the pre-version, post-version, and return value are all equal. We know, for any observed read with a defined return value, exactly what version it observed.

Writes are more complicated, because it may be the case that multiple writes could have resulted in a given version. For example, consider two observed increment operations $\hat{w}_1 = w(\_, 1) \xrightarrow{} (\_, nil)$ and $\hat{w}_2 = w(\_, 1) \xrightarrow{} (\_, nil)$. Which of these writes (and therefore, which transaction) resulted in the version 2? It could be \textit{either} $\hat{w}_1$ or $\hat{w}_2$. We cannot construct a single dependency graph for this observation--though we could construct a (potentially exponentially large) set of dependency graphs, and check each one for cycles.

What if we had an observation which allowed us to uniquely determine the observed write which produced a given version? We say an observation $O$ is \textit{recoverable} iff, for every write $w$ in the set of all writes implied by the traces of all versions observed by committed reads, $w$ has exactly one compatible write in $O$.

There are several ways to obtain recoverable histories. For instance, we could define our writes such that, like reads, each returns the version it produced; e.g. for increments, $w_x(3, 1) \xrightarrow{} (4, 4)$. This approach works when all return values are known. However, an indeterminate transaction could result in a write which is committed in some interpretations, but whose return value is unknown. Having multiple such writes could make it impossible to tell which resulted in a given version.

Another possibility is to limit the number of writes. If we perform at most one write to every object, for instance, there is no question about which observed write was responsible for an object's one and only state transition.

Perhaps the most useful approach to obtaining recoverability is to enforce the following five constraints on an observation $O$. Two are choices we can make in generating histories: we can choose to work with traceable objects, and use a unique argument for every write performed. The remaining three are behaviors that well-behaved databases should exhibit---and which can be detected should they fail to hold. Committed reads should be consistent with one another, which gives us a single trace of writes to consider. Since arguments are distinct per object $x$ in $O$, so they should be distinct in the trace of $x_{longest}$ as well. Finally, versions shouldn't pop into existence magically; every committed version we read should be the product of some sequence of writes in $O$.

\begin{lemma}
An observation $O$ is recoverable if all of the following hold:

\begin{enumerate}
    \item Every $x$ in $O$ is traceable.
    \item No pair of $(x, a)$ appears more than once in the writes in $O$.
    \item $O$ is consistent.
    \item Every argument $a$ in the trace of $x_{longest}$ is distinct.
    \item Every write in the trace of $x_{longest}$ has a compatible write in $O$.
\end{enumerate}
\end{lemma}

\begin{proof}
Consider an object $x$ in $O$. Since $x$ is traceable and $O$ is consistent, the trace of every committed read of $x$ is a prefix of the trace of $x_{longest}$. To show recoverability, we must prove that every write in the trace of $x_{longest}$ has exactly one compatible write in $O$, for all $x$.

Consider a single write $w = (x_i, a) \xrightarrow{} (x_j, r)$ in the trace of $x_{longest}$. Per (4), $a$ is unique in that trace. Per (5), there exists at least one write $\hat{w} = w(_, \hat{a}) \xrightarrow{} (_, \hat{r})$ in $O$ which is compatible with $w$. Since $w$ and $\hat{w}$ are compatible, $\hat{a} = a$. Per (2), there is no other write of $a$ to $x$ in $O$. This implies $\hat{w}$ is the \textit{only} compatible write for $w$ in $O$.
\end{proof}




\subsection{Detecting Dirty Updates and Aborted Reads}

We can use these definition of compatibility, along with properties of traceable objects and recoverable observations, to infer whether or not an observation implies dirty reads or aborted updates.

Imagine we record an observation $O$ from some database system where all objects are traceable. We wish to know whether that system exhibited anomalies---but anomalies are properties of \textit{histories}, not observations. We would like to prove that certain types of anomalies are present in every interpretation of $O$, or that there exists at least one interpretation which has no anomalies.

Consider the set $X_c$ of versions of $x$ read by committed transactions in some observation $O$. We denote a single version with a trace longer than any other $x_{longest}$---if there are multiple longest traces, any will do. We say $O$ is \textit{consistent} if for all $x$ in $O$, every $x_i \in X_c$ is in the trace of $x_{longest}$. Otherwise, $O$ is \textit{inconsistent}.

\begin{lemma}
\label{inconsistent->aborted-read}
If an observation $O$ is inconsistent, every interpretation of $O$ exhibits aborted reads.
\end{lemma}

\begin{proof}
If $O$ is inconsistent, then there exists a committed read $r_i$ of some version $x_i$ which is not in the trace of $x_{longest}$. If $x_i$ is aborted, then $r_i$ is an aborted read by definition. Likewise, if $x_{longest}$ is not committed, then our committed read of $x_{longest}$ is an aborted read.

If, on the other hand, both $x_i$ and $x_{longest}$ are committed, then consider lemma \ref{traceable->x_max-trace-all-committed}, which states that every committed version of $x$ must be in the trace of $x_{max}$. This means both $x_i$ and $x_{longest}$ are in the trace of $x_{max}$.

Since $x_i$ is not in the trace of $x_{longest}$, $x_{longest}$ must be in the trace of $x_i$---but this would imply $x_i$ is both observed by a committed read, and has a longer trace than $x_{longest}$, which contradicts the definition of $x_{longest}$. Therefore $x_i$ must be aborted, and $r_i$ is an aborted read.
\end{proof}

\begin{lemma}
\label{traceable+recoverable+aborted-write-immediately-before-read->aborted-read}
If a traceable, recoverable observation $O$ has a committed read of version $x_i$, which, (by recoverability) was the product of a write $\hat{w}_i$, and the transaction $\hat{T}_i$ containing $\hat{w}_i$ is aborted, then every interpretation of $O$ exhibits aborted read.
\end{lemma}

\begin{proof}
Consider an interpretation $(H, R)$ of $O$. By compatibility with $O$, $H$ contains a committed read of $x_i$. By traceability, there is exactly one write $w_i$, in transaction $T_i$, which produced $x_i$. Recoverability implies that there is exactly one transaction ($\hat{T}_i$) in $O$ which is compatible with $T_i$. Since $\hat{T}_i$ aborted, $T_i$ aborted as well. $x_i$ is therefore the product of an aborted write, which satisfies the definition of an aborted read.
\end{proof}

\begin{lemma}
\label{traceable+recoverable+aborted-write-before-committed-write-before-read->dirty-update}
If a traceable, recoverable observation $O$ has a committed read of some version $x_k$ with at least two versions $x_i$ and $x_j$ in the trace of $x_k$, in that order, and recoverability implies that the transaction $\hat{T}_i$ which wrote $x_i$ aborted, and the transaction $\hat{T}_j$ committed, then every interpretation of $O$ exhibits dirty update.
\end{lemma}

\begin{proof}
Analogous to lemma \ref{traceable+recoverable+aborted-write-immediately-before-read->aborted-read}, every interpretation $(H, R)$ of $O$ contains an aborted version $x_i$ and a committed version $x_j$, such that a path exists between $x_i$ and $x_j$ in $v_x$. By traceability, this path is unique. Therefore there must exist some write between $x_i$ and $x_j$ which takes an uncommitted version to a committed one: a dirty update.
\end{proof}

\begin{lemma}
\label{traceable+recoverable+aborted-write-before-read->dirty-update-or-aborted-read}
If a traceable, recoverable observation $O$ has a committed read of some $x_j$, and some write $w_i$ in the trace of $x_j$ belongs (via recoverability) to an aborted transaction in $O$, then every interpretation of $O$ exhibits either an aborted read or a dirty update.
\end{lemma}

\begin{proof}
Consider an interpretation $(H, R)$ of $O$. If $x_j$ is aborted in $H$, then the committed read of $x_j$ in $O$ implies a corresponding committed read of $x_j$ in $H$: an aborted read.

If $x_j$ is committed in $H$, then there must exist some write $w_j$ which produced $x_j$ and committed in $H$. Since $w_i$ aborted in $O$ (and therefore in $H$ as well), $w_i \neq w_j$, and $w_i$ must precede $w_j$ in the trace of $x_j$. Lemma \ref{traceable+recoverable+aborted-write-before-committed-write-before-read->dirty-update} tells us that $H$ must contain a dirty update.
\end{proof}

Traceability and recoverability allow us to map observed transactions to the traces of committed reads. If we observe an aborted write whose consequences are reflected in a committed read, we know that either an aborted read or a dirty update has taken place (or that no histories exist at all). If we know the committed or aborted status of the transaction which produced the value we read, or we can find a committed write between the two, we can distinguish between dirty updates and aborted reads.

\subsection{Detecting Intermediate Reads}

Given a history $H$, Adya et al define an intermediate read (G1b) as a committed transaction $T_j$ which reads a version of object $x$ written by a transaction $T_i$, which was not $T_i$'s final modification of $x$. Given an observation $O$, can we say whether all interpretations $(H, R)$ of $O$ exhibit intermediate reads? In general, we cannot: an observation may not tell us what actual \textit{versions} were produced by a given write. However, for traceable objects, we can infer, from a read, exactly which updates produced which versions. Recoverability, in turn, lets us identify whether those updates were intermediate or final in their respective transactions.

\begin{lemma}
\label{intermediate-read}
Given a recoverable observation $O$ of a database with a traceable object $x$, if $O$ contains a committed transaction $\hat{T}_j$ which reads $x_i$, and the trace of $x_i$ implies, via recoverability, that $x_i$ was the product of an intermediate write in some observed transaction $\hat{T}_i$, then every interpretation $(H, R)$ of $O$ contains an intermediate read.
\end{lemma}

\begin{proof}
Since $\hat{T}_j$ is committed, its corresponding transaction $T_j$ in every $H$ must be committed too. Likewise, $T_i$'s write of $x_i$ must not be $T_i$'s final write of $x$, in order to be compatible with $\hat{T}_i$. By recoverability, and the fact that $R$ is bijective, $T_i \neq T_j$. Therefore, every $H$ has an intermediate read.
\end{proof}





\subsection{Inferred Version Orders}

Consider an observation $O$ of a database where all objects are traceable, and an interpretation $(H, R)$ of $O$. We wish to show that we can derive $H$'s version order $\ll$ from $O$ alone, with minimal constraints on $H$ and $R$. Lemma \ref{x_i->ll_x-prefix} allows us to recover a prefix of $\ll_x$ from any installed $x_i$ in $H$, assuming we know which transactions in the trace of $x_i$ committed, and which aborted. In order to know which versions are committed or aborted, we assume $H$ must not contain aborted reads, intermediate reads, or dirty updates. We call these \textit{clean} interpretations.

Given an observation $O$, which installed version of $x$ should we use? Ideally, we would have $x_{max}$. However, some writes leading to $x_{max}$ may be unobserved. Instead, we take a version $x_f$ read by a transaction $\hat{T}_f$ such that:

\begin{itemize}
    \item $\hat{T}_f$ is committed.
    \item $\hat{T}_f$ read $x_f$ before performing any writes to $x$.
    \item No other version of $x$ satisfying the above properties has a longer trace than $x_f$.
\end{itemize}

It would also be possible to take $x_{longest}$ and unwind/advance history to the nearest installed version, but this approach complicates the proof, and is not required for soundness.

\begin{lemma}
\label{x_f-is-installed}
If $O$ is an observation, and $(H, R)$ is an interpretation of $O$ which has neither aborted reads nor intermediate reads, $x_f$ is an installed version in $H$.
\end{lemma}

\begin{proof}
Since $O$ contains a transaction $\hat{T}_f$ reading $x_f$, there must be a compatible $T_f$ in $H$ which is also committed and read $x_f$ before performing any writes to $x$. Since $T_f$ is committed, and $H$ has neither intermediate nor aborted reads, we know that $x_f$ must have been the result of a final write by some committed transaction in $H$.
\end{proof}

\begin{lemma}
\label{x_f-trace-is-all-committed}
If $O$ is an observation, and $(H, R)$ is a clean interpretation of $O$, then every version in the trace of $x_f$ was written by a committed transaction in $H$.
\end{lemma}

\begin{proof}
Some of the transactions in the trace of $x_f$ might be indeterminate in $O$. However, we know from lemma \ref{x_f-is-installed} that $x_f$ is an installed (and therefore committed) version. If an uncommitted write \textit{were} in the trace of $x_f$, then there must exist a committed transaction which performed a write on top of uncommitted state. This would constitute a dirty update: a contradiction. Therefore, every version in the trace of $x_f$ was written by a committed transaction in $H$.
\end{proof}

\begin{lemma}
\label{obs->ll-prefix}
If $O$ is an observation, and $(H, R)$ is a clean interpretation of $O$, then for every object $x$ in $O$, removing intermediate versions from the trace of $x_f$ yields $<_x$: the prefix of $\ll_x$ up to and including $x_f$.
\end{lemma}

\begin{proof}
Lemma \ref{x_f-is-installed} tells us that $x_f$ is an installed version in $H$, and lemma \ref{x_f-trace-is-all-committed} tells us that every version in the trace of $x_f$ was written by a committed transaction in $H$. Lemma \ref{x_i->ll_x-prefix} states that removing intermediate and aborted versions from the trace of $x_f$ yields the prefix of $\ll_x$ up to and including $x_f$. We know this trace has no aborted versions, so all that must be done is to remove intermediate versions.
\end{proof}

Note that these lemmata hold regardless of our specific choice of $(H, R)$. Given any observation, we can reconstruct a prefix of $\ll_x$ which holds for \textit{all} clean interpretations.

As a final step, we define an \textit{inferred version order} $<$ by combining the prefix chains from lemma \ref{obs->ll-prefix}: $< \: \equiv \: <_x \cup <_y \cup \ldots$, where $<_x \cup <_y$ means the chain whose members are the union of members in $<_x$ and $<_y$, and whose order is the union of orders in $<_x$ and $<_y$.

\subsection{Inferred Serialization Graphs}

Given a recoverable observation $O$ of a database of traceable objects, we can infer a chain of versions $<$. Recoverability also allows us to map every version in $<$ to a particular write in $O$ which produced it. Using these, we define \textit{inferred dependencies} between pairs of transactions $\hat{T}_i$ and $\hat{T}_j$ in $O$ as follows:

\begin{itemize}
    \item \textbf{Direct inferred write-write dependency}. A transaction $\hat{T}_j$ \textit{directly inferred-ww-depends} on $\hat{T}_i$ if $\hat{T}_i$ performs a final write of a version $x_i$ of $x$, and $\hat{T}_j$ performs a final write resulting in $x$'s next version $x_j$, by $<$.
    
    \item \textbf{Direct inferred write-read dependency}. A transaction $\hat{T}_j$ \textit{directly inferred-wr-depends} on $\hat{T}_i$ if $\hat{T}_i$ performs a final write of a version $x_i$ in $<$, and $\hat{T}_j$ reads $x_i$.
    
    \item \textbf{Direct inferred read-write dependency}. A transaction $\hat{T}_j$ \textit{directly inferred-rw-depends} on $\hat{T}_i$ if $\hat{T}_i$ reads version $x_i$ of $x$, and $\hat{T}_j$ performs a final write of $x$'s next version in $<$.
\end{itemize}

Unlike Adya et al's definitions, we don't require that a transaction \textit{install} some $x_i$, because an indeterminate transaction in $O$ might be committed in \textit{interpretations} of $O$, and have corresponding dependency edges there. Instead, we rely on the fact that $<$ only relates installed versions in clean interpretations.

An \textit{Inferred Direct Serialization Graph}, or \textit{IDSG}, is a graph of dependencies between observed transactions. The IDSG for an observation $O$ is denoted IDSG($O$). If $\hat{T}_j$ inferred-ww-depends on $\hat{T}_i$, there exists an edge labeled \textit{ww} from $\hat{T}_i$ to $\hat{T}_j$ in IDSG($O$), and similarly for inferred-wr and inferred-rw-dependencies.

8We would like to show that for every clean interpretation of an observation, the IDSG is (in some sense) a subgraph of the DSG. However, the IDSG and DSG are graphs over different types of transactions; we need the bijection $R$ to translate between them. Given a relation $R$ and a graph $G$, we write $R \diamond G$ to denote $G$ with each vertex $v$ replaced by $Rv$.

\begin{theorem}
\label{IDSG-subgraph-of-DSG}
For every clean interpretation $(H, R)$ of an observation $O$, $R \diamond IDSG(O)$ is a subgraph of $DSG(H)$.
\end{theorem}

\begin{proof}
It suffices to show that every edge in $R \diamond IDSG(O)$ is also in $DSG(H)$. We consider a pair of observed transactions $\hat{T}_i$ and $\hat{T}_j$ in $O$, and their corresponding transactions in $H$: $T_i = R \hat{T}_i$ and $T_j = R \hat{T}_j$.

\begin{itemize}
\item[ww] If $\hat{T}_j$ directly inferred-ww-depends on $\hat{T}_i$, then $T_j$ directly ww-depends on $T_i$.

\begin{proof}
Per the definition of inferred-ww-depends, $\hat{T}_i$ performed a final write of some version $x_a$, and $\hat{T_j}$ performed a final write of some $x_b$, such that $x_a$ immediately precedes $x_b$ in $<$. By lemma \ref{obs->ll-prefix}, $<_x$ is a prefix of $\ll_x$, which means $x_a$ also directly precedes $x_b$ in $\ll$. Since $\ll$ relates installed versions, $x_a$ and $x_b$ are both installed. Recoverability ensures that there is only one write in $O$ which could produce $x_a$ (and $x_b$, respectively). Since $R$ relates compatible transactions, $T_i = R \hat{T}_i$, and likewise for $T_j$. Since $x_a$ directly precedes $x_b$ in $\ll$, and $T_i$ installed $x_a$, and $T_j$ installed $x_b$, $T_j$ directly ww-depends on $T_i$.
\end{proof}

\item[wr] If $\hat{T}_j$ directly inferred-wr-depends on $\hat{T}_i$, then $T_j$ directly wr-depends on $T_i$.

\begin{proof}
By the definition of inferred-wr-depends, $\hat{T}_i$ performs a final write of a version $x_i$ in $<$, and $\hat{T}_j$ reads $x_i$. Since $x_i$ is in $<$, it is committed in $H$. Compatibility & recoverability imply that $T_i$'s write producing $x_i$ was final; $T_i$ therefore installs $x_i$ in $H$. Compatibility implies $T_j$ read $x_i$. Therefore, $T_i$ directly wr-depends on $T_j$.
\end{proof}

\item[rw] If $\hat{T}_j$ directly inferred-rw-depends on $\hat{T}_i$, then $T_j$ directly rw-depends on $T_i$.

\begin{proof}
By the definition of inferred-rw-depends, $\hat{T}_i$ contains a read of $x_i$ and $\hat{T}_j$ performs a final write of $x_j$, such that $x_i$ immediately precedes $x_j$ in $<$. Via $R$, $T_i$ also contains a read of $x_i$. By recoverability, $T_j$ also performs a final write of $x_j$. Since $<$ contains $x_j$, $T_j$ must have committed, which means $T_j$ installed $x_j$. By lemma \ref{obs->ll-prefix}, $<_x$ is a prefix of $\ll_x$, which means $x_i$ directly precedes $x_j$ in $\ll$ as well. Therefore, $T_j$ directly rw-depends on $T_i$.
\end{proof}
\end{itemize}

Since every edge $\hat{T}_i \xrightarrow{} \hat{T}_j$ in $IDSG(O)$ has a corresponding edge $T_i \xrightarrow{} T_j$ in $DSG(H)$, $R \diamond IDSG(O)$ is a subgraph of $DSG(H)$.
\end{proof}

\subsection{Inferred Anomalies}

Theorem \ref{IDSG-subgraph-of-DSG} tells us that every cycle in IDSG($O$) has a corresponding cycle in every clean interpretation of $O$. For every anomaly defined in terms of cycles on a DSG (e.g. G1c, G2, G-single, G2-item, \ldots), we can define a corresponding anomaly on an IDSG. If we detect that anomaly in IDSG($O$), its corresponding anomaly must be present in every clean interpretation of $O$ as well!

Of course, this result only applies to \textit{clean} interpretations. What of unclean interpretations, like those with aborted reads or dirty updates? If those occurred, the trace of a version read by a committed transaction could cause us to infer a version order $<_x$ which includes uncommitted versions, and is not a prefix of $\ll_x$. A clean interpretation could have cycles absent from an unclean interpretation, and vice versa.

This is not as bad as one might think. Lemma \ref{inconsistent->aborted-read} and \ref{traceable+recoverable+aborted-write-before-read->dirty-update-or-aborted-read} tell us that aborted reads and dirty updates are, in some cases, detectable. Moreover, the more determinate transactions an observation contains, the more likely we are to detect those anomalies.

Phenomena like aborted reads and dirty updates are, in a very loose sense, "worse" than dependency cycles like G1c and G2. If every interpretation of an observation must exhibit aborted reads, the question of whether it also exhibits anti-dependency cycles is not as pressing! And if some interpretations exist which \textit{don't} contain aborted reads, but all of those exhibit anti-dependency cycles, we can choose to give the system the benefit of the doubt, and say that it definitely exhibits G2, but may not exhibit aborted reads.

==> sketch.tex <==
We begin our proof by defining a model of a database, transactions, and histories, closely adapted from Adya et al. We omit predicates for simplicity, and generalize Adya's read-write registers to objects supporting arbitrary transformations as writes, resulting in a \textit{version graph}. We constrain Adya's \textit{version order $\ll$} to be compatible with this version graph. This generalization introduces a new class of anomaly: \textit{dirty updates}.

We define write-write, read-write, and write-read dependencies between transactions, adapted directly from Adya's formalism, as well as a \textit{direct serialization graph} using those dependencies. The anomalies we wish to find are expressed in terms of that serialization graph.

We go on to define a class of \textit{traceable objects}, which permit recovery of the version graph and object operations resulting in any particular version, and show that list-append objects are traceable. We use traceability to recover the version order $\ll$ from any committed version in a history.

When we interact with a database system, the history may not be accessible from outside the database---or perhaps no "real" history exists at all. We define an \textit{observation} of a system as a set of experimentally-accessible transactions where versions, return values, and committed states may be unknown, and consider the \textit{interpretations} of that observation--the set of all histories which could have resulted in that particular observation.

\paa{still left to cannibalize}
We show that traceability allows us to (sometimes) detect when every interpretation of an observation would exhibit aborted reads, dirty updates, or intermediate reads. If we consider \textit{clean interpretations} which do not exhibit those anomalies, we can use any committed read of an object to derive a prefix of the version order for that object $\ll_x$ which must hold in every interpretation. Using that version order prefix, we construct an \textit{inferred direct serialization graph}, which is a subgraph of the direct serialization graph for every interpretation. We can use that graph to identify anomalies, like G-single, which must be present in every clean interpretation of a given observation.
